An Asynchronous Distributed-Memory Parallel Algorithm for k-mer Counting

This paper describes a new asynchronous algorithm and implementation for the problem of k-mer counting (KC), which concerns quantifying the frequency of length k substrings in a DNA sequence. This operation is common to many computational biology workloads and can take up to 77% of the total runtime of de novo genome assembly. The performance and scalability of the current state-of-the-art distributed-memory KC algorithm are hampered by multiple rounds of Many-To-Many collectives. Therefore, we develop an asynchronous algorithm (DAKC) that uses fine-grained, asynchronous messages to obviate most of this global communication while utilizing network bandwidth efficiently via custom message aggregation protocols. DAKC can perform strong scaling up to 256 nodes (512 sockets / 6K cores) and can count k-mers up to 9x faster than the state-of-the-art distributed-memory algorithm, and up to 100x faster than the shared-memory alternative. We also provide an analytical model to understand the hardware resource utilization of our asynchronous KC algorithm and provide insights on the performance.

==> REMOVED-FROM--intro.tex <==
\begin{comment}
    arguably the most common kernel in all of computational genomics.
    High throughput DNA/RNA/protein sequencing is an essential part of fundamental life science research and clinical diagnostics. 
    \kc is arguably the most common kernel is all of computational genomics.
    %Applications of \kc include
\end{comment}

\begin{comment}
    both as standalone tools~\cite{hysortk,kmerindsc18} and as part of genome assembly pipelines~\cite{hipmer,pakman,metahipmer}.
\end{comment}
    
\begin{comment}
    A na\"ive approach to counting \kmers would use a standard dictionary with each distinct \kmer value as the key and its frequency (count) as the corresponding value. %, and keeping track of all possible \kmers observed in the input datasets. 
    But, thanks to the drastic reduction in the cost of sequencing technologies, the amount of data generated by sequencing experiments has far outpaced the improvement of a single processor's computational power.
    That makes the dictionary approach of counting \kmers computationally prohibitive for counting billions of \kmers from massive datasets, often observed in real life.
    Given the myriad of applications supported by \kc, there has been abundant research towards developing faster and more memory efficient \kc algorithms~\cite{kmc2,kurtz_new_2008,li_mspkmercounter:_2015,li2018gpu,mamun_kcmbt_2016,marcais_fast_2011,pan2018optimizing,pandey2018squeakr,rizk_dsk:_2013} on shared memory processors.
    For instance, KMC3, a widely used shared memory \kmer counter, requires about 2.5 hours, 34 GB RAM, and 500 GB disk space on a sequence of 729 Gbp~\cite{kmc3}.
    The practical alternative is designing distributed memory parallel \kc algorithms that can utilize the vast amount of memory and computational resources available in a modern supercomputer.
    % A fundamentally different approach to \kc will be to build distributed memory parallel \kc algorithms that can utilize the vast amount of memory and computational resources available in modern supercomputers, to count \kmers from massive datasets significantly faster.
    Significant efforts have been spent on designing distributed memory \kc algorithms, both as standalone tools~\cite{hysortk,kmerindsc18} and as part of genome assembly pipelines~\cite{hipmer,pakman,metahipmer}.
    Yet, \kmer counting takes up to 77\% time on a short-read genome assembly pipeline PakMan~\cite{pakman}.
    Even, GPU-accelerated metagenome assembly tool MetaHipMer2~\cite{mhmgpu} spends to 50\% of the total runtime just doing \kmer analysis.
    This makes \kc the primary bottleneck in a lot of genomics workloads.
    % , and make it essential to design faster distributed memory \kc algorithms.
    
    The two main challenges of \kc are poor data locality and load imbalance, the latter of which derives from the inherently skewed \kmer distributions that appear in real biological datasets and are only detectable at runtime. 
    %
    % This makes it essential to design faster distributed memory \kc algorithms.
    % The challenges in \kc stem from the fact that the amount of data generated by sequencing experiments is massive, and the amount of compute per unit data access, and data reuse is very low.
    % The added challenge comes from real-world biological datasets that have inherently skewed distribution of \kmers, posing additional load balancing issues.
\end{comment}

% Two popular distributed memory \kc algorithms are HySortK~\cite{hysortk} and KmerInd~\cite{kmerindsc18} that employed parallel sorting and AVX2 based hash tables respectively to count \kmers from massive datasets in parallel.
% But both the attempts are limited by their \BSP based design that forces the algorithms to perform multiple rounds collectives, limiting the algorithm's performance and scalability.

% eof

==> genomics.tex <==
\subsection{Short-read genome assembly}
Talk about PakMan and HipMer
\subsection{Long-read genome assembly}
Talk about HySortK and ELBA
\subsection{Metagenome assembly}
Talk about multiple rounds of \kmer counting in MetaHipMer
